Tensor Algebra and its Applications to Data Science and Statistics

This survey provides an overview of common applications, both implicit and explicit, of "tensors" and "tensor products" in the fields of data science and statistics. One goal is to reconcile seemingly distinct usages of the term "tensor" in the literature, and to explain how these usages are manifestations of a common concept. Not all relevant topics are discussed in detail, but the attempt is made to briefly describe and give references for some of the most important topics not included in the main survey. Particular attention is given to tensor decompositions.

==> multilinear/rank.tex <==
In \cite{Kruskal1989}, the multiplex rank corresponding to slices ("slabs") is introduced as the "dimensionality vector". The author then notes that for third order tensors ("three-way arrays") the multilinear rank, i.e. the multiplex rank corresponding to the hyperslice family (fibers) dual to the slices, gives the same ranks, a special case of the result stated above, with the same proof given. (Namely that matricization of the tensor with one of the fibers as one of the modes of the matrix necessarily implies that the dual hyperslices, i.e. the slices/slabs, are the other mode of the matrix, and then applying the fact that row rank equals column rank for any matrix.) Upper and lower bounds, similar to those found in \cite{Diaz2016}, on the rank of a third order tensor in terms of the multilinear and multiplex ranks are also given in \cite{Kruskal1989}, namely that, for a third order-tensor $\mathbfcal{T}$ with multiplex rank (or equivalently multilinear rank) $(R, S,T)$, both $\operatorname{rank}(\mathbfcal{T}) \ge \max\{R,S,T\}$ and $\operatorname{rank}(\mathbfcal{T}) \le \min \{ RS, RT, ST\}$.

==> symmetric_tensors.tex <==

\section{Permutations of Modes and Symmetric Tensors}
\label{sec:perm-modes-symm}

The very imprecise statement that ``$\mathcal{U} \otimes \mathcal{T}$ will always have the same entries as $\mathcal{T} \otimes \mathcal{U}$ but in different places'', is easiest to make precise in the case of vectors and matrices. Specifically, given a vector $\mathbf{v} \in \mathbb{R}^M$ and a vector $\mathbf{w} \in \mathbb{R}^N$, it follows from the definitions that:
\[  \mathbf{w} \otimes \mathbf{v} = (\mathbf{v} \otimes \mathbf{w})^\top \,,  \]
where $^\top$ denotes the operation of matrix transposition. The above allows us to define matrix transposition as a function on rank-one tensors. In fact, the function $(\mathbf{v},\mathbf{w}) \mapsto \mathbf{w} \otimes \mathbf{v}$ is bilinear, so the universal property of the tensor product allows us to extend this definition for elementary tensors (in this case rank-one matrices in $\mathbb{R}^{[M] \times [N]}$) to a linear function defined on all tensors (matrices in $\mathbb{R}^{[M] \times [N]}$). Thus, using the universal property of the tensor product, matrix transposition can be defined as follows: given a matrix $A \in \mathbb{R}^{[M] \times [N]}$, and some arbitrary decomposition of $A$ into a linear combination of elementary tensors, 

\[  A = \sum_{i=1}^I a_i \mathbf{v}_i \otimes \mathbf{w}_i \,,  \]

where $I \ge 1, \text{ and for all }i \in [I], a_i \in \mathbb{R}, \mathbf{v}_i \in \mathbb{R}^M, \mathbf{w}_i \in \mathbb{R}^N$, then the transpose of $A$ is:

\[  A^\top = \sum_{i=1}^I a_i \mathbf{w}_i \otimes \mathbf{v}_i \,.  \]
Notice how the vectors $\mathbf{v}_i \in \mathbb{R}^M$ correspond to the first mode of $A$ and the second mode of $A^\top$, whereas the vectors $\mathbf{w}_i\in \mathbb{R}^N$ correspond to the second mode of $A$ and the first mode of $A^\top$. Thus matrix transposition corresponds to transposing the two modes of a second order tensor. 

Similarly, for any two tensors $\mathcal{T}$ and $\mathcal{U}$, one can recover $\mathcal{T} \otimes \mathcal{U}$ from $\mathcal{U} \otimes \mathcal{T}$, and vice versa, via a suitable permutation of the modes. (Note that while $\mathcal{T} \otimes \mathcal{U}$ and $\mathcal{U} \otimes \mathcal{T}$ may have different shapes, they will always have the same order.) What it means to permute the modes of a tensor has not been defined precisely above, but is entirely analogous to the example given above.

While the above definition of matrix transposition looks like it might depend on the chosen way of writing $A$ as a linear combination of elementary tensors, the universal property of the tensor product guarantees that it does not. Here are two concrete examples of this. Letting $\mathbf{e}_w^{(W)}$ denote the unit vectors in $\mathbb{R}^W$, and given $A \in \mathbb{R}^{[H] \times [W]}$ letting $A_{:w} \in \mathbb{R}^H$ denote the columns of $A$, then we can write $A$ as the following linear combination of elementary tensors:
\[ A = \sum_{w=1}^W A_{:w} \otimes \mathbf{e}_w^{(W)} \,, \]
which means, using the above definition of matrix transposition, that:
\[  A^\top = \sum_{w=1}^W \mathbf{e}_w^{(W)} \otimes A_{:w} \,, \]
or in other words that the columns of $A$ are the rows of $A^\top$. Similarly, letting $\mathbf{e}_h^{(H)}$ denote the unit vectors in $\mathbb{R}^H$, and $A_{h:} \in \mathbb{R}^W$ denote the rows of $A$, then we can also write $A$ as the following linear combination of elementary tensors:
\[  A = \sum_{h=1}^H e_{h}^{(H)} \otimes A_{h:} \,, \]
which means, using the above definition of matrix transposition, that:
\[ A^\top = \sum_{h=1}^H A_{h:} \otimes e_{h}^{(H)} \,,  \]
or in other words that the rows of $A$ are the columns of $A^\top$. While these two possible definitions of $A^\top$ may seem possibly contradictory, that the columns of $A^\top$ are the rows of $A$, or that the rows of $A^\top$ are the columns of $A$, the universal property of the tensor product is what guarantees that these two definitions describe the same operation.

A matrix $A$ is called a symmetric matrix if and only if $A^\top = A$. As discussed above, this is equivalent to saying that the matrix remains the same after permuting its two modes. Analogously, a general tensor is called\footnote{Note that (cite Kolda and Bader) break with conventional practice and call such tensors ``supersymmetric''.} a \textbf{symmetric tensor} if and only if it remains the same after any permutation of its modes. Any symmetric matrix is square, for obvious reasons, and for the analogous reason any symmetric tensor is cubical.

In fact symmetric tensors, because their modes can be permuted arbitrarily, are essentially ``commutative'', and therefore correspond exactly to homogeneous polynomials. There are several, inter-related ways to make this precise, but giving the background required to explain them is outside the scope of this review.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "new_notes_draft"
%%% End:

